Learning Neural Acoustic Fields

Our environment is filled with rich and dynamic acoustic information. When we walk into a cathedral, the reverberations as much as appearance inform us of the sanctuary's wide open space. Similarly, as an object moves around us, we expect the sound emitted to also exhibit this movement. While recent advances in learned implicit functions have led to increasingly higher quality representations of the visual world, there have not been commensurate advances in learning spatial auditory representations. To address this gap, we introduce Neural Acoustic Fields (NAFs), an implicit representation that captures how sounds propagate in a physical scene. By modeling acoustic propagation in a scene as a linear time-invariant system, NAFs learn to continuously map all emitter and listener location pairs to a neural impulse response function that can then be applied to arbitrary sounds. We demonstrate that the continuous nature of NAFs enables us to render spatial acoustics for a listener at an arbitrary location, and can predict sound propagation at novel locations. We further show that the representation learned by NAFs can help improve visual learning with sparse views. Finally, we show that a representation informative of scene structure emerges during the learning of NAFs.

==> figtext/lin_probe.tex <==
\begin{figure}[!t]
  \centering
  \vspace{-0.5em}
  \includegraphics[width=0.9\linewidth]{figure/linear_probe.pdf}
\vspace{-5pt}
  \caption{\small \textbf{Qualitative Visualization of scene structure decoding with a linear layer.} \textbf{Top:} The ground truth scene structure map, at each position we visualize the distance to the nearest wall. \textbf{Middle:} Linear decoding results using MFCC features. \textbf{Bottom:} Linear decoding results using NAF features.}

  \label{fig:linearmap}
\end{figure} 

==> figtext/tsne.tex <==
\begin{figure}[!t]
  \centering
  \vspace{-8pt}
  \includegraphics[width=0.9\linewidth]{figure/tsne_plot.pdf}
\vspace{-5pt}
  \caption{\small \textbf{Visualization of NAF latents.} We apply TSNE to reduce the dimensionality of the NAF latents. The latents learned by our NAF exhibit clear structure.}
  \label{fig:tsnemap}
\end{figure} 

==> text/07_checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope? \answerYes{}
  \item Did you describe the limitations of your work? \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work? \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them? \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)? \answerYes{} See repo provided on site. 
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)? \answerYes{}.
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{} We use a single fixed seed for all our experiments.
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNo{} We utilize public datasets only.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{} Does not apply to our data.
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerYes{} Was not determined to create any risks.
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNo{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> text/08_impact.tex <==
\section{Societal Impact} Our work focuses on learning a high quality representation of acoustic fields. The primary use case for our work lies in virtual reality and gaming. As our work can lead to more believable and higher quality representations of spatial audio than alternative methods, it is possible that our work could increase the dependency and time spent on gaming. The more compact nature of our acoustic representations may allow for spatial audio to be deployed to more systems, and enable more equitable access.
